WebRobot: Web Robotic Process Automation using Interactive Programming-by-Demonstration

It is imperative to democratize robotic process automation (RPA), as RPA has become a main driver of the digital transformation but is still technically very demanding to construct, especially for non-experts. In this paper, we study how to automate an important class of RPA tasks, dubbed web RPA, which are concerned with constructing software bots that automate interactions across data and a web browser. Our main contributions are twofold. First, we develop a formal foundation which allows semantically reasoning about web RPA programs and formulate its synthesis problem in a principled manner. Second, we propose a web RPA program synthesis algorithm based on a new idea called speculative rewriting. This leads to a novel speculate-and-validate methodology in the context of rewrite-based program synthesis, which has also shown to be both theoretically simple and practically efficient for synthesizing programs from demonstrations. We have built these ideas in a new interactive synthesizer called WebRobot and evaluate it on 76 web RPA benchmarks. Our results show that WebRobot automated a majority of them effectively. Furthermore, we show that WebRobot compares favorably with a conventional rewrite-based synthesis baseline implemented using egg. Finally, we conduct a small user study demonstrating WebRobot is also usable.

==> impl.tex <==
\vspace{-7pt}
\section{Implementation}
\label{sec:impl}
\vspace{-0pt}

We have implemented our proposed ideas in a new tool called \toolname. It is a Chrome extension with a frontend and a backend. The backend implements our synthesis algorithm and consists of 5000 lines of TypeScript code. The frontend is written in JavaScript, CSS, and HTML, primarily implementing our interface. We used Express.js from Node.js as our middleware framework for communications between the frontend and backend. 
More implementation details can be found in Appendix~\ref{appendix:impl} (supplemental). 

\begin{comment}


In what follows, we discuss some key optimizations and heuristics in our implementation. 


\vspace{1pt}
\textbf{\em Bounded space of alternative selectors.}
While our DSL (Figure~\ref{fig:dsl}) allows arbitrary nesting of $\domchildren$ and $\domdescendants$ operators, our implementation considers up to two levels of nesting (e.g., $\domchildren$ inside $\domdescendants$). In addition, we also allow using full XPath expressions. This is shown to be quite useful in practice, without significantly sacrificing expressiveness. 

\vspace{1pt}
\textbf{\em Sampling constant selectors.}
Even if we consider a smaller space of alternative selectors, there could still be hundreds of them per action, which makes our parametrization process slow (e.g., \emph{R1} in Figure~\ref{fig:parametrize}).  Our implementation randomly samples 5 constant selectors when parametrizing actions. 


\vspace{1pt}
\textbf{\em Synthesizing multiple programs.}
While it returns only one program from Algorithm~\ref{alg:top}, our implementation returns multiple programs whose predictions are then visualized in the frontend. Users can navigate within these predictions. 

\vspace{1pt}
\textbf{\em Phase transition heuristics.}
We have a few heuristics for transitioning across phases. For instance, we transition from the authorization phase if multiple programs all have the same prediction (which means there is no ambiguity). 

\end{comment}




==> semantics.tex <==
\newcounter{mycounter}

\begin{figure*}[!t]
%\small 
\footnotesize
%\scriptsize 
\begin{centermath}
\centering
\begin{array}{cc}
\irule{
\begin{array}{c}
\statetrace = \bot 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\block_1; \dots; \block_m
}{
\bot, \bot, \bot 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\statetrace = \emptylist
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\block_1; \dots; \block_m
}{
\emptylist, \emptylist, \env 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
m \geq 2 \ \ \ \ 
\evalprogram{
\actiontrace, \statetrace, \env
}{
\block_{1}
}{
\actiontrace', \statetrace', \env' 
} \ \ \ \ 
\evalprogram{
\actiontrace \statetraceminus \actiontrace', \statetrace \statetraceminus \statetrace', \env'
}{
\block_{2}; \dots; \block_m 
}{
\actiontrace\doubleprime, \statetrace\doubleprime,  \env\doubleprime
}
\\ 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\block_1; \dots; \block_m  
}{
\actiontrace' \actiontraceconcat \actiontrace\doubleprime, \statetrace' \statetraceconcat \statetrace\doubleprime,  \env\doubleprime
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\action' = \clickaction(\xpath) \ \ \ \ 
(  \actiontrace', \statetrace', \env') = \left\{
\begin{array}{ll}
( [\action'], [\mystate_1],  \env ) & \consistent(\action', \actiontrace) \\ 
( \bot, \bot, \bot ) & \emph{otherwise} \\ 
\end{array}
\right. 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace,  \env
}{
\clickinstruction(\domnode)
}{
\actiontrace', \statetrace', \env'
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\action' = \gobackaction \ \ \ \ 
( \actiontrace', \statetrace', \env' ) = \left\{
\begin{array}{ll}
( [\action'], [\mystate_1], \env ) & \consistent(\action', \actiontrace) \\ 
( \bot, \bot, \bot ) & \emph{otherwise} \\ 
\end{array}
\right.
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\gobackinstruction}{
}{
\actiontrace', \statetrace', \env' }
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\action' = \scrapetextaction(\xpath) \\ 
( \actiontrace', \statetrace', \env') = \left\{
\begin{array}{ll}
( [\action'], [\mystate_1], \env ) & \consistent(\action', \actiontrace) \\ 
( \emptylist, \emptylist, \env ) & \neg\consistent(\action', \actiontrace) \land \neg\valid(\xpath, \mystate_1 ) \\ 
( \bot, \bot, \bot ) & \emph{otherwise} \\ 
\end{array}
\right.
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\scrapetextinstruction(\domnode)
}{
\actiontrace', \statetrace', \env'
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\action' = \sendkeysaction(\xpath, \conststring) \\ 
( \actiontrace', \statetrace', \env') = \left\{
\begin{array}{ll}
( [\action'], [\mystate_1], \env ) & \consistent(\action', \actiontrace) \\ 
( \bot, \bot, \bot ) & \emph{otherwise} \\ 
\end{array}
\right.
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\sendkeysinstruction(\domnode, \conststring)}{
\actiontrace', \statetrace', \env' 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\evalinputvalue{\env}{\inputvalue}{\inputvaluepath} \ \ \ \ 
\action' = \senddataaction(\xpath, \inputvaluepath) \\ 
(\actiontrace', \statetrace', \env') = \left\{
\begin{array}{ll}
( [\action'], [\mystate_1],  \env ) & \consistent(\action', \actiontrace) \\ 
( \bot, \bot, \bot ) & \emph{otherwise} \\ 
\end{array}
\right.
\end{array}
}{
\evalprogram{ \actiontrace, \statetrace, \env}{\senddatainstruction(\domnode, \inputvalue)}{\actiontrace', \statetrace', \env' }
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evalprogram{
\actiontrace, \statetrace, \env
}{
\foreach{\domnodevar}{\domnodes_{\geq 1}}{ \program } 
}{
\actiontrace', \statetrace', \env' 
}
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\foreach{\domnodevar}{\domnodes}{ \program } 
}{
\actiontrace', \statetrace', \env' 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnodes_{\geq i}}{\xpath \listconcat \domnodes'_{\geq i+1}} \ \ \ \ 
\neg\valid( \xpath, \mystate_1 ) 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\foreach{\domnodevar}{\domnodes_{\geq i}}{ \program } 
}{
\emptylist, \emptylist, \env
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnodes_{\geq i}}{\xpath \listconcat \domnodes'_{\geq i+1}} \ \ \ \ 
\valid( \xpath, \mystate_1 ) \\ 
\evalprogram{
\actiontrace, \statetrace, \env[ \domnodevar \mapsto \xpath ]
}{
\program; \foreach{\domnodevar}{\domnodes'_{\geq i+1}}{ \program } 
}{
\actiontrace', \statetrace', \env'
}
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env
}{
\foreach{\domnodevar}{\domnodes_{\geq i}}{ \program } 
}{
\actiontrace', \statetrace', \env' 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evalinputvalues{\env}{\inputvalues}{ [ \inputvaluepath_1, \dots, \inputvaluepath_m ] } \ \ \ \ 
\actiontrace_1 = \actiontrace \ \ \ \ 
\statetrace_1 = \statetrace \ \ \ \ 
\env_1 = \env[\inputvaluevar \mapsto \inputvaluepath_1] \ \ \ \ 
\evalprogram{\actiontrace_1, \statetrace_1, \env_1}{\program}{\actiontrace'_1, \statetrace'_1, \env'_1} \\ 
\actiontrace_{i} = \actiontrace_{i-1} \traceminus \actiontrace'_{i-1} \ \ \ \ 
\statetrace_{i} = \statetrace_{i-1} \traceminus \statetrace'_{i-1} \ \ \ \ 
\env_{i} = \env'_{i-1}[\inputvaluevar \mapsto \inputvaluepath_i] \ \ \ \ 
\evalprogram{\actiontrace_i, \statetrace_i, \env_i}{\program}{\actiontrace'_i, \statetrace'_i, \env'_i} \ \ \ \ 
2 \leq i \leq m 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace, \env}{
\foreach{\inputpathvar}{\inputvalues}{\program} 
}{
\bigtraceconcat^{m}_{i=1} \actiontrace'_i, 
\bigtraceconcat^{m}_{i=1} \statetrace'_i, 
\env'_m
}
} & (\showmycounter{mycounter})
\\ \\ 
\irule{
\begin{array}{c}
\evalprogram{
\statetrace, \actiontrace, \env[ \intvar \mapsto i ]}{
\program; 
\textbf{\texttt{if}} \ \valid(\domnode) \ \textbf{\texttt{do}} \ \big\{ 
\clickinstruction(\domnode); 
\foreachint{\intvar \geq i+1}
{ 
\{ \program; \clickinstruction(\domnode) \} \big\}
} 
}{
\actiontrace', \statetrace', \env' 
}
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace,  \env}{
\foreachint{\intvar \geq i}
{
\{
\program; 
\clickinstruction(\domnode) 
\} 
} 
}{
\actiontrace', \statetrace', \env' 
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\neg\valid(\xpath, \mystate_1) 
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace,  \env}{
\textbf{\texttt{if}} \ \valid(\domnode) \ \textbf{\texttt{do}} \ \program
}{
\emptylist, \emptylist, \env
}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\statetrace = [ \mystate_1, \dots, \mystate_m ] \ \ \ \ 
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\valid(\xpath, \mystate_1) \ \ \ \ 
\evalprogram{\actiontrace, \statetrace, \env}{\program}{\actiontrace', \statetrace', \env'}
\end{array}
}{
\evalprogram{
\actiontrace, \statetrace,  \env}{
\textbf{\texttt{if}} \ \valid(\domnode) \ \textbf{\texttt{do}} \ \program
}{
\actiontrace', \statetrace', \env'
}
} & (\showmycounter{mycounter})
\end{array}
\end{centermath}
\caption{Semantics.}
\end{figure*}








\resetmycounter{mycounter}

\begin{figure*}[!t]
%\small 
\footnotesize
%\scriptsize 
\begin{centermath}
\centering
\begin{array}{cc}
\irule{
\begin{array}{c}
\end{array}
}{
\evaldomnode{\env}{\xpath}{\xpath}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\end{array}
}{
\evaldomnode{\env}{\domnodevar}{\env[\domnodevar]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\evalpredicate{\env}{\predicate}{\xpathpredicate} \\ 
\end{array}
}{
\evaldomnode{\env}{
\domnode/\predicate[i]
}{\xpath/\xpathpredicate[i]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\evalpredicate{\env}{\predicate}{\xpathpredicate} \\ 
\end{array}
}{
\evaldomnode{\env}{
\domnode\sslash\predicate[i]
}{\xpath\sslash\xpathpredicate[i]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\end{array}
}{
\evalpredicate{\env}{\domtag}{\domtag}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\end{array}
}{
\evalpredicate{\env}{\domtag[\domattribute=\conststring]}{\domtag[\domattribute=\conststring]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\conststring = \env[\inputvaluevar]
\end{array}
}{
\evalpredicate{\env}{
\domtag[\textattribute=\inputvaluevar]
}{\domtag[\textattribute=\conststring]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
k = \env[\intvar]
\end{array}
}{
\evalpredicate{\env}{\domtag[\textattribute=\intvar]}{\domtag[\textattribute=k]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\evalpredicate{\env}{\predicate}{\xpathpredicate} \\ 
\end{array}
}{
\evaldomnodes{\env}{\domchildren( \domnode, \predicate)_{\geq i}}{\xpath\slash\xpathpredicate[i] \listconcat \domchildren( \xpath, \xpathpredicate)_{\geq i+1} }
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evaldomnode{\env}{\domnode}{\xpath} \ \ \ \ 
\evalpredicate{\env}{\predicate}{\xpathpredicate} \\ 
\end{array}
}{
\evaldomnodes{\env}{\domdescendants( \domnode, \predicate)_{\geq i}}{\xpath\sslash\xpathpredicate[i] \listconcat \domdescendants( \xpath, \xpathpredicate)_{\geq i+1} }
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\end{array}
}{
\evalinputvalue{\env}{\inputvaluevar}{\env[\inputvaluevar]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evalinputvalue{\env}{\inputvalue}{\inputvaluepath}
\end{array}
}{
\evalinputvalue{\env}{\inputvalue[\emph{key}]}{\inputvaluepath[\emph{key}]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evalinputvalue{\env}{\inputvalue}{\inputvaluepath}
\end{array}
}{
\evalinputvalue{\env}{\inputvalue[i]}{\inputvaluepath[i]}
} & (\showmycounter{mycounter})
\\ 
\\ 
\irule{
\begin{array}{c}
\evalinputvalue{\env}{\inputvalue}{\inputvaluepath} \ \ \ \ 
\emph{arr} =  \emph{GetArray} ( \inputdata, \inputvaluepath  )
\end{array}
}{
\evalinputvalues{\env}{\inputchildren(\inputvalue)}{ \big[ \inputvaluepath[1], \dots, \inputvaluepath[|\emph{arr}|] \big] }
} & (\showmycounter{mycounter})
\end{array}
\end{centermath}
\caption{Semantics.}
\end{figure*}






